Tower of Babel in Cross-Cultural Communication: A Case Study of #Give Me a Chinese Name# Dialogues During the "TikTok Refugees'' Event

The sudden influx of "TikTok refugees'' into the Chinese platform RedNote in early 2025 created an unprecedented, large-scale online cross-cultural communication event between the West and East. Although prior HCI research has studied user behavior in social media, most work remains confined to monolingual or single-cultural contexts, leaving cross-linguistic and cultural dynamics underexplored. To address this gap, we focused on a particularly challenging cross-cultural encoding-decoding task that remains stubbornly beyond the reach of machine translation, i.e., foreign newcomers asking Chinese users for Chinese names, and examined how people collectively constructed a digital "Babel Tower'' through various information encoding strategies. We collected and analyzed over 70,000 comments from RedNote with a creative human-in-the-loop approach using large language models, deriving a systematic framework summarizing cross-cultural information encoding strategies, how they are combined and layered to complicate decoding, and how they relate to engagement metrics such as the number of likes.

==> ACMprocess-metadata.tex <==
\title{Tower of Babel in Cross-Cultural Communication: A Case Study of \#Give Me a Chinese Name\# Dialogues During the "TikTok Refugees" Event}

\author{Jielin Feng}
\orcid{0009-0008-1943-5609}
\affiliation{
\department{School of Data Science}\institution{Fudan University}
\city{Shanghai}
\country{China}}
\email{23110980031@m.fudan.edu.cn}

\author{Zhibo Yang}
\orcid{0009-0006-9679-5101}
\affiliation{
\department{School of Journalism}\institution{Fudan University}
\city{Shanghai}
\country{China}}
\email{22300130030@m.fudan.edu.cn}

\author{Jingyi Zhao}
\orcid{0009-0006-7355-5519}
\affiliation{
\department{School of Foreign Language and Literature}\institution{Fudan University}
\city{Shanghai}
\country{China}}
\email{22300120121@m.fudan.edu.cn}

\author{Yujia Li}
\orcid{0009-0003-8846-8889}
\affiliation{
\department{School of Journalism}\institution{Fudan University}
\city{Shanghai}
\country{China}}
\email{23301170062@m.fudan.edu.cn}

\author{Xinwu Ye}
\orcid{0009-0008-3164-0373}
\affiliation{\institution{Fudan University}
\city{Shanghai}
\country{China}}
\affiliation{
\department{School of Computing and Data Science}\institution{The University of Hong Kong}
\city{Hong Kong}
\country{China}}
\email{xinwuye43@connect.hku.hk}

\author{Xingyu Lan}
\orcid{0000-0001-7331-2433}
\affiliation{
\department{School of Journalism}\institution{Fudan University}
\city{Shanghai}
\country{China}}
\email{xingyulan96@gmail.com}

\author{Siming Chen}
\orcid{0000-0002-2690-3588}
\affiliation{
\department{School of Data Science}\institution{Fudan University}
\city{Shanghai}
\country{China}}
\affiliation{
\department{Qingdao Research Institute}\institution{Fudan University}
\city{Shanghai}
\country{China}}
\email{simingchen3@gmail.com}
